ABN: Anti-Blur Neural Networks for Multi-Stage Deformable Image Registration

Deformable image registration, i.e., the task of aligning multiple images into one coordinate system by non-linear transformation, serves as an essential preprocessing step for neuroimaging data. Recent research on deformable image registration is mainly focused on improving the registration accuracy using multi-stage alignment methods, where the source image is repeatedly deformed in stages by a same neural network until it is well-aligned with the target image. Conventional methods for multi-stage registration can often blur the source image as the pixel/voxel values are repeatedly interpolated from the image generated by the previous stage. However, maintaining image quality such as sharpness during image registration is crucial to medical data analysis. In this paper, we study the problem of anti-blur deformable image registration and propose a novel solution, called Anti-Blur Network (ABN), for multi-stage image registration. Specifically, we use a pair of short-term registration and long-term memory networks to learn the nonlinear deformations at each stage, where the short-term registration network learns how to improve the registration accuracy incrementally and the long-term memory network combines all the previous deformations to allow an interpolation to perform on the raw image directly and preserve image sharpness. Extensive experiments on both natural and medical image datasets demonstrated that ABN can accurately register images while preserving their sharpness. Our code and data can be found at https://github.com/anonymous3214/ABN

==> 05_experiment.tex <==
%\section{Experiment and Analysis}
\section{Experiments}
\label{section:Experiments}

\subsection{Datasets} \label{section:Dataset}
%In order to evaluate our proposed ABN method, we conduct experiments on both natural and medical image registration tasks, by using the following datasets.
In order to evaluate the performance of our method on image registration tasks, we conduct experiments on three different datasets, one with natural images (2D) and two with medical images (3D).

\noindent\textbullet\ \textit{Flickr-Faces-HQ (FFHQ)} \cite{karras2019style}: 
%This dataset is extracted from FFHQ,
We used a subset of the FFHQ dataset, which contains 400 human face images, randomly sampled from the whole dataset. 
%Following \cite{dai2020dual}, we collect the pairs of source images and target images by applying random transformations to the raw image. 
In order to construct pairs of source and target images, similar to \cite{dai2020dual}, we random transform each face image using a random deformation field. % smoothed by a Gaussian filter. 
%We then use the original and deformed image pairs as the target and source images, respectively, and form them in a pair. 
We use the deformed image as the target image and the raw image as the source image. We resize all images to $64\times64$, and randomly split the image pairs into training and test sets with the ratio of 80$\%$ and 20$\%$, respectively. 

\noindent\textbullet\ \textit{LPBA40} \cite{shattuck2008construction}: 
This dataset consists of 40 T1-weighted 3D brain MRI scans and the corresponding segmentation ground truth of 56 anatomical structures. 
The ground truth is used to evaluate the registration accuracy. 
Same as \cite{balakrishnan2018unsupervised, zhao2019recursive}, we focus on atlas-based registration in this experiment, in which the first scan in the dataset is the target image and the remaining scans need to be aligned with the target image. 
Among the 39 scans,  30 scans are used for training and 9 scans are used for testing. 
All scans are resized to $96\times96\times96$ after cropping.

\noindent\textbullet\ \textit{MindBoggle101} \cite{klein2012101}: 
This dataset contains 101 T1-weighted 3D brain MRI scans and the corresponding annotation of 25 cortical regions, but only 62 scans have their valid segmentation ground truth. 
Following the recent work \cite{liu2019probabilistic}, we focus on atlas-based registration using 41 scans for training and 20 scans for testing. All scans are resized to $96\times96\times96$ after cropping.


% \noindent\textbullet\ \textbf{Face Image:}
% For the 2D face image registration, we use FFHQ (Flickr-Faces-HQ) \cite{karras2019style} dataset which contains 70,000 human face images. Similar to the approach use in \cite{dai2020dual}, we collect the pairs of source images and target images by applying random transformations to the raw image. We first dealigned each image using a random deformation field smoothed by a Gaussian filter. We then take the original image and the dealigned image as the target image and source image respectively, and paced them in a pair. We randomly select 400 pairs of images and divided them into one group of 320 and the other group of 80 for training and test. Finally, all images are resized to $64\times64$.

% \noindent\textbullet\ \textbf{Brain MRI:} We use two public datasets for the 3D brain MRI registration, LPBA40 \cite{shattuck2008construction} and MindBoggle101 \cite{klein2012101}. LPBA40 consists of 40 T1-weighted scans and the corresponding segmentation ground truth of 56 anatomical structures. The ground truth is used to evaluate the registration accuracy. Same as \cite{balakrishnan2018unsupervised, zhao2019recursive}, we focused on atlas-based registration in this experiment, in which the first scan in LPBA40 
% is a target image and the rest of the scans need to align with it. Among the rest 39 scans, a group of 30 scans and the other group of 9 scans were used for training and testing, respectively. MindBoggle101 contains 101 T1-weighted scans and the corresponding annotation of 25 cortical regions, but only 62 scans have their valid segmentation ground truth. Following the recent work \cite{liu2019probabilistic}, we used 42 images for training and 20 images for testing. All scans of two datasets were resized to $96\times96\times96$ after cropping.
\input{tab_methods_v4}

\subsection{Compared Methods}
\label{section:Compared Methods}
We compare our approach to seven state-of-the-art methods, as shown in Table~\ref{tab:methods}.

\noindent\textbullet\ \textit{Affine registration (Affine)} \cite{avants2009advanced}: 
This method breaks the image registration task into a composition of a linear transformation and a translation. 
% Affine mapping would suffice the task when only translation, rotation, scaling and shearing are needed. We used existing affine implementation in the publicly available software package - ANTs \cite{avants2009advanced}.

\noindent\textbullet\ \textit{BSpline transform (BSpline)} \cite{rueckert1999nonrigid}: This method uses control points and spline functions to describe the nonlinear geometric transformation domain.

\noindent\textbullet\ \textit{Demons algorithm (Demons)} \cite{thirion1998image}: This method is inspired by the optical flow equations and considers non-rigid image registration as a diffusion process.

\noindent\textbullet\ \textit{Elastic registration (Elastic)} \cite{bajcsy1989multiresolution,avants2009advanced}: This method estimates the elastic geometric deformation by updating transformation parameters iteratively. 
% The Elastic is included in ANTs \cite{avants2009advanced} software package. We ran the elastic registration with the default setting.


\noindent\textbullet\ \textit{Symmetric normalization (SyN)} \cite{avants2008symmetric}: This is a top-performing traditional method for deformable image registration \cite{klein2009evaluation, balakrishnan2018unsupervised}. This method optimizes the space of diffeomorphic maps by maximizing the cross-correlation between images. 
% Same as Elastic, we ran SyN via ANTs \cite{avants2009advanced} with a default setting.


\noindent\textbullet\ \textit{VoxelMorph (VM)} \cite{balakrishnan2018unsupervised}: This is an unsupervised single-stage registration method, which use one network to predict the deformation between images.

% For network architectures, we used the latest version, VoxelMorph-2, and configured 10 convolutional layers with 16, 32, 32, 64, 64, 64, 32, 32, 32 and 16 filters.

\noindent\textbullet\ \textit{Cascaded Registration Networks (CRN)} \cite{zhao2019recursive}:
This is a state-of-the-art method for unsupervised image registration with a multi-stage design. In different stages, the source image is repeatedly deformed to align with a target image.

% In terms of the setting of convolutional layers and filters of each stage, CRN is the same as VM.


\noindent\textbullet\ \textit{Anti-Blur Networks (ABN)}:
This is our proposed model which consists of two sub-networks at each stage, the short-term registration and long-term memory networks. 

\noindent\textbullet\ \textit{Anti-Blur Networks-Long (ABN-L)}: ABN-L is a variant of ABN, which only contains a long-term memory network $f_{L}(\cdot, \cdot)$ at each stage. The network handle the registration and combination of deformations simultaneously.

% ABN-L is our proposed method with a lightweight architecture. Each stage of the method contains only one sub-registration network to predict the deformation field. As introduced in Section \ref{sec:ABN-L}, each sub-registration network has 3 inputs, thus we configured 10 convolutional layers of the sub-registration network with 32, 64, 64, 128, 128, 128, 64, 64, 64 and 32 filters. The number of stages of ABN-L is the same as that of CRN for fair comparison. 


% The number of convolutional layers in both sub-registration network is the same as that of VM and CRN. Again, to ensure a fair comparison, the number of stages of ABN is the same as that of CRN and ABN-L.


\subsection{Evaluation Metrics}
We use two metrics to assess the registered image quality: registration accuracy and image sharpness, which are detailed as follows. 
% Due to the differences between datasets used in the two tasks, separate evaluation metrics are used to assess the registration accuracy. 
% The 3D brain MRI datasets include the segmentation of anatomical structures that can be used to measure registration performance. However, the 2D face image dataset only contains different pairs of source images and target images. Thus their registration accuracy can only be evaluated by the similarity between the final warped images and the target images. Therefore, we use corresponding evaluation metrics for each task. 
% We introduce each corresponding evaluation metric in the following subsection.
\input{fig_res_2d}
\input{tab_2d}

\subsubsection{Registration Accuracy}
\label{section:Registration accuracy}
%\hphantom{1}
%\newline
%\noindent\textbullet\ \textbf{2D face registration:} 
% As introduced in the previous section,
The 2D face dataset only contains the pairs of source and target images. To evaluate the registration accuracy, we measure the image similarity by cross-correlation (CC) \cite{rabiner1978digital} and structural similarity (SSIM) \cite{wang2004image} between the final warped image and the target image.

%\noindent\textbullet\ \textbf{3D brain MRI registration:} 
The brain MRI datasets contain the segmentation ground truth of anatomical structures, which is location labels of different tissues in the brain. If the two images are well-aligned, then their anatomical structures should overlap with each other. Thus, it is reasonable to use the structure overlap between the final warped image and the target image to evaluate the registration performance. Similar to \cite{balakrishnan2018unsupervised,zhao2019recursive,de2019deep}, we used Dice score and Jaccard coefficient to measure the overlap between two structures (warped and target).
% , which can be formulated as:
% \begin{equation}
% {\displaystyle Dice(X,Y)={\frac {2|X\cap Y|}{|X|+|Y|}}}  
% \end{equation}
% \begin{equation}
% \operatorname{Dice}(\mathbf{S}_{w}, \mathbf{S}_{t})=2 \cdot \frac{|\mathbf{S}_{w} \cap \mathbf{S}_{t}|}{|\mathbf{S}_{w}|+|\mathbf{S}_{t}|}
% \end{equation}
% where
% \begin{equation}
% \mathbf{S}_{w}=\mathcal{T}\left(\mathbf{S}_{s}, \phi\right).
% \end{equation}
% $\mathbf{S}_{s}$, $\mathbf{S}_{t}$ and $\mathbf{S}_{w}$ are structural segmentation of the source image, target image and warped image, respectively. $\phi$ is the predicted deformation field. 
%The final score is the average dice score for each anatomical structure.
The final score is the average of the dice score of the each structure.

\input{fig_face_stage_v2}

\subsubsection{Image Sharpness}
%\hphantom{1}
%\newline
%\indent 
We quantify the sharpness of the final warped image by Sum Modulus Difference (SMD) \cite{santos1997evaluation} and Tenengrad \cite{yeo1993autofocusing,tenenbaum1970accommodation}. Those are popular no-reference sharpness evaluation metrics.
% SMD evaluated the sharpness of an image by calculating the difference between the values of each pixel and its neighboring pixels. 
SMD evaluated the sharpness of an image by summing the differences between adjacent pixels. If the image is sharp, then we expect the difference is larger than that of a blurred image. 
% %We used SMD to measure the difference between neighboring pixels, which can be computed as:
% \begin{equation}
% \begin{split}
% \operatorname{SMD}(\mathbf{I}_{w})=\sum_{x}^{W} \sum_{y}^{H} \sum_{z}^{D}|\mathbf{I}_{w}(x+1, y, z)-\mathbf{I}_{w}(x, y, z)| \\
% +|\mathbf{I}_{w}(x, y+1, z)-\mathbf{I}_{w}(x, y, z)|
% +|\mathbf{I}_{w}(x, y, z+1)-\mathbf{I}_{w}(x, y, z)|
% \end{split}
% \end{equation}
% where $\mathbf{I}_{w}(x, y, z)$ is the voxel value of the warped image $\mathbf{I}_{w}$ at the 3D coordinate $(x, y, z)$. $W$, $H$ and $D$ represent the width, height and depth of the image, respectively.
Tenengrad evaluated the sharpness of an image by extracting its edge information. The image edge is the region where the intensity of the image signal changes rapidly, and the sharper the image, the faster the edge changes. 

% We used Tenengrad, a edge-based metric, to measure the sharpness of image, which can be defined as:
% \begin{multline}
% \operatorname{Tenengrad}(\mathbf{I}_{w})=\sum_{n}^{W} \sum_{m}^{H} \sum_{l}^{D} \Big(\mathbf{G}_{x}^{2}(n,m,l) \\
% +\mathbf{G}_{y}^{2}(n,m,l)+\mathbf{G}_{z}^{2}(n,m,l)\Big)
% \end{multline}
% where $\mathbf{G}_{x}$, $\mathbf{G}_{y}$ and $\mathbf{G}_{z}$ are respectively the gradients of the horizontal, vertical, and axial directions, computed using Sobel operators \cite{sobel1972camera}. 

\subsection{Experiment Setting.}
We split the datasets into training and test sets as described in the Datasets section. 
For 2D face registration, models are trained with batch size of 16 for 5$k$ epochs. 
For 3D brain MRI registration, we reduce the batch size to 1 to address GPU memory limitation and models were trained for 1$k$ epochs. 
For both tasks, models are optimized using Adam optimizer~\cite{kingma2014adam} with a learning rate of $1 \times 10^{-4}$. 
The ratios of regularization in Eq.~\eqref{eq:loss} is set to $\lambda=10$.
For more details, please refer to Appendix~\ref{sec:appendix}. The source code is available at \url{https://github.com/anonymous3214/ABN}.


\subsection{Experimental Results}
We evaluate the proposed method in 2D face registration and 3D brain MRI registration tasks. For each task, we quantify the performance of registration accuracy and the image sharpness by their corresponding metrics. Across all of these metrics, we find that ABN achieves higher registration accuracy and image sharpness than the state-of-the-art methods.

%Before we go to details we would first like to highlight two important findings in our performance evaluation:

%\noindent \textbf{Superior performance of ABN}: Across all of these metrics, we find that ABN achieves higher registration accuracy and image sharpness than the state-of-the-art methods. 

%\noindent \textbf{Handling vanishing details:} In the study of parameter influence, we gradually increase the number of stages. The registration accuracy of multi-stage baseline CRN first increases and then drops dramatically. In the contrast, our proposed ABN shows a continuing increasing curve. The result provides a strong evidence to show the ``vanishing details'' problem of multi-stage registration. Also, it supports the effectiveness of our proposed ABN.  
% Implementation details and code are available in the supplementary material.
% All models were implemented using PyTorch with the code available at 
\input{tab_3d_v4}
\input{fig_para_3d}
% described in Section \ref{section:Compared Methods}.
% \vspace{-5}
\subsubsection{Results on 2D Face Registration}
% \hphantom{1}
% \newline
%\indent 
Table~\ref{tab:2D res} summarizes the results of four methods on 2D face registration task. It can be seen that ABN clearly outperforms all the baselines in terms of both registration accuracy (SSMI and CC) and image sharpness (SMD and Tenengrad). We observed a gain in SSMI of roughly $3.8\%$ and in SMD up to $9.9\%$ compared to the best baseline method CRN.
Notably, the registration accuracy of ABN-L is lower than that of ABN since ABN-L only contains a long-term memory network, which is insufficient for obtaining a high quality registration result.
% Compared to the best performing baseline CRN, ABN improves the registration accuracy by $3.8\%$ in SSMI and increases the image sharpness by $9.9\%$ in SMD. 
% CRN achieves slightly better registration accuracy relative to our another proposed method ABN-L. However, ABN-L performs significantly better in preserving image sharpness than CRN.


Figure \ref{fig:face result} shows visual comparisons of 2D face registration results. Upon inspection, we can see that the final warped image of ABN is more similar to the target image than those of VM, CRN and ABN-L. Most notably, in terms of sharpness, ABN-L and ABN clearly outperform CRN. VM does not appear to have a loss in sharpness, but it is significantly worse than other methods in registration accuracy. Furthermore, we also compare the intermediate warped results of our method with other multi-stage method (\ie CRN), as shown in Figure \ref{fig:face stage}. It is clear that both methods allow the warped/registered images to progressively align to the target image with the help of a multi-stage fashion. However, the registration accuracy improvement of CRN is accompanied by a loss of image sharpness, while ABN gives much sharper images than CRN.

\subsubsection{Results on 3D Brain MRI Registration}
%\hphantom{1}
%\newline
%\indent 
Table \ref{tab:3D res} shows the results of nine methods on two respective datasets: LPBA40 and Mindboggle101.
% The performances of Affine, BSpline, Demons, Elastic, SyN, VM and CRN are compared with our methods - ABN-L and ABN.
%The run time is measured on the same device with a Intel$^{\circledR}$ Xeon$^{\circledR}$ E5-2667 v4 CPU and a NVIDIA Tesla V100 GPU. No GPU implementations of BSpline, Demons, Elastic and SyN have been found in previous works \cite{yaniv2018simpleitk,avants2009advanced,bajcsy1989multiresolution,avants2008symmetric,balakrishnan2018unsupervised,zhao2019recursive}.
In this task, Dice score and Jaccard are used to evaluate registration accuracy, while SMD and Tenengrad are used to assess sharpness performance.
The results of each method are shown with its average performance with standard deviation and its ranking among all other methods.
Based on the global competition in both datasets, the average ranking of ABN outperforms that of all baselines. 
Specifically, ABN achieves superior performance against all compared methods on registration accuracy, while achieving competitive results in image sharpness persevering.
We observe that almost all multi-stage methods outperform the single-stage methods on registration accuracy, but only ABN-L and ABN are on par with single-stage methods in terms of image sharpness persevering.
Again, the overall performance of ABN-L was slightly inferior to that of ABN, indicating that the short-term registration network is crucial and beneficial to improve registration accuracy.
% In order to evaluate our proposed methods, we compared them with several competitive approaches: Affine, BSpline, Demons, Elastic and SyN for traditional iteration-based methods, VM and CRN for deep learning based approaches. 
% In this task, we used Dice score and Jaccard coefficient to assess the performance of the registration accuracy. The run time is measured on the same device with a Intel$^{\circledR}$ Xeon$^{\circledR}$ E5-2667 v4 CPU and a NVIDIA Tesla V100 GPU. No GPU implementations of BSpline, Demons, Elastic and SyN have been found in previous works \cite{yaniv2018simpleitk,avants2009advanced,bajcsy1989multiresolution,avants2008symmetric,balakrishnan2018unsupervised,zhao2019recursive}.

% As shown in Table \ref{tab:3D res}, again, ABN achieves image sharpness on par with the best method (VM) and the highest registration accuracy than any other alternative state-of-the-art method. Specifically, compared to the best performing learning-based method CRN, ABN improves the registration accuracy by $4.3\%$ in Dice score and increases the image sharpness by $20\%$ in SMD. In this task, the other method proposed by us, ABN-L also outperforms all of the baselines in terms of registration accuracy, and has a close performance to VM in sharpness preservation. VM has achieved the best result for image sharpness preservation, but is inferior to our proposed methods in registration accuracy. For traditional iteration-based methods, Elastic achieves a result closest to ABN-L, but proves to be much more time-consuming. Though Affine produces competitive result in image sharpness preservation, it is significantly worse in registration accuracy.

Figure \ref{fig:brain result} shows the visual comparisons of one sample of the 3D brain MRI registration task on the LPBA40 dataset. We can observe that our ABN method is more accurate in aligning the source image to the target image. Notably, although CRN has an impressive performance in registration accuracy, the warped registered image is obviously blurred, which can be verified with the focused example of the anatomical structure. 
%The Affine only performs a global linear transformation, so its performance is significantly worse than other nonlinear-based registration methods in terms of registration accuracy. 
Although single-stage methods (Affine, BSpline, Demons, Elastic, SyN, and VM) involve only one interpolation and o dnot suffer from image blurring problem, they are inferior to the multi-stage methods (CRN, ABN-L and ABN) in terms of registration performance.
These results indicate that our proposed method effectively achieves a higher level of registration accuracy while preserving image sharpness.

We also compared the registration speed among the traditional and learning-based methods, as shown in Figure~\ref{fig:time}. To clearly show the time of all baselines in the chart, we omitted method Demons, which takes the longest time for registration: 100.95 seconds on the Mindboggle 101 dataset and 81.98 seconds on the LPBA40 dataset. Upon observation, it is clear that all traditional methods consumes much more time compared to learning-based methods. Specifically, all learning-based methods can achieve real-time registration within one second. Compared with the most accurate non-learning method Elastic, our proposed ABN achieves even higher accuracy and only uses 2.5\% time of Elastic. 
\input{fig_res_3d}
%We also compared the registration speed among the traditional and learning based method. The one of the important reasons to use neural networks in image registration is to achieve real-time speed. As we can see in Figure~\ref{fig:time}, the traditional methods for deformable registration, i.e. BSpline, Elastic and SyN requires significant longer time than the neural network methods VM, CRN and ABN. Compared with the most accurate non-learning method Elastic, our proposed ABN achieves even higher accuracy and only uses 2.5\% time of Elastic.  

\subsubsection{Influence of Parameters.}
% In this subsection, we study the performance of all multi-stage methods with different stage numbers in 3D brain MRI registration. 
We study the performance of all multi-stage methods at different stage number settings using the LPBA40 dataset.
For multi-stage methods, the number of stages corresponds to the depth of the network and the number of warping operations. In other words, more stages mean more refinements of the alignment, which is usually beneficial to the improvement of registration accuracy. However, a larger number of stages also consumes more GPU memory and increase the computation time. To investigate the influence of different stage settings, we compared 10 different versions of the CRN, ABN-L, and ABN, with the number of stages varies from 1 to 10.
% \indent For the 2D face registration task, as shown in Figure \ref{fig:2D SSMI} and Figure \ref{fig:2D CC}, ABN achieves the highest registration accuracy, especially when the number of stages is large, e.g., greater than 5, ABN outperforms all other methods. When assessing sharpness of registered images, it can be seen from Figure \ref{fig:2D SMD} and Figure \ref{fig:2D Tenengrad} that ABN and ABN-L consistently superior to CRN at any stage. We found that the image sharpness of CRN was consistent with the increase of the number of stages in this task. The reason is that CRN always perform the transformation from previous registered image. When the image is distorted in the previous stage, it can cause irreparable damage in the subsequent stages. In this case, further stages no longer affect the performance even the number of stages increased, resulting in registration accuracy and image sharpness remaining constant. 
% % A visualization of the example results can be found in the appendix.

As illustrated in Figure \ref{fig:3D Dice}, both ABN-L and ABN significantly outperform CRN in the registration accuracy as the number of stages increases. In addition, ABN-L and ABN consistently preserve the image sharpness, as observed in Figures \ref{fig:3D SMD} and \ref{fig:3D Tenengrad}. Notably, in this task, the effectiveness of CRN in both registration accuracy and image sharpness decreases significantly when the number of stages increases. This supports our intuition that recursively deforming the image obtained
from the previous stage will result in image blurring and signal attenuation, which causes the registration accuracy to further deteriorate. Thus, our methods ABN-L and ABN outperform CRN in the multi-stage case in both registration accuracy and sharpness preserving.

==> fig_face_stage.tex <==
\begin{figure}[t]
    \centering
    \subfigure[\textbf{CRN}]{
        \includegraphics[width=0.98\linewidth]{fig/face_stage_1.pdf}
        \label{fig:stage 1}
    }
    \subfigure[\textbf{ABN (ours)}]{
        \includegraphics[width=0.98\linewidth]{fig/face_stage_2.pdf}
        \label{fig:stage 2}
    }
    \caption{Comparing the intermediate and final results of different multi-stage methods in 2D face image registration. We use the 10-stage CRN and ABN as examples to demonstrate the performance of registration at each stage.}
    \label{fig:face stage}
    %\vspace{-10pt}
\end{figure}

==> fig_network1.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/network_1_v3.pdf}
  \caption{Overview of unsupervised end-to-end learning for image registration.}
  \label{fig:unsupervised}
\end{figure}



==> fig_para_2d.tex <==
\begin{figure*}[t]
    \centering
    \subfigure[Registration accuracy by SSMI]{
        \includegraphics[width=0.23\textwidth]{fig/2Dface_SSMI.pdf}
        \label{fig:2D SSMI}
    }
    \subfigure[Registration accuracy by CC]{
        \includegraphics[width=0.23\textwidth]{fig/2Dface_CC.pdf}
        \label{fig:2D CC}
    }
    \subfigure[Sharpness by SMD]{
        \includegraphics[width=0.23\textwidth]{fig/2Dface_SMD.pdf}
        \label{fig:2D SMD}
    }
    \subfigure[Sharpness by Tenengrad]{
        \includegraphics[width=0.23\textwidth]{fig/2Dface_Tenengrad.pdf}
        \label{fig:2D Tenengrad}
    }
    \caption{Performance of multi-stage methods with different number of stages on 2D face registration task.}
    \label{fig:2D parameters}
\end{figure*}

==> tab_datasets.tex <==
\begin{table}[h]
    \centering
    \caption{Summary of datasets}
    \label{tab:dataset}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
     & \textbf{FFHQ}& \textbf{LPBA40 }& \textbf{Mindboggle101}\\
    \midrule
    Domain  & Natural & Medical & Medical\\
    Subject  & Face RGB& Brain MRI& Brain MRI\\
    Dimension &  2D & 3D & 3D\\
    Image size & $64\times64$  & $96\times96\times96$ & $96\times96\times96$\\
    Sample size & 400 & 40 & 62\\
    \bottomrule
    \end{tabular}}
\end{table}


==> tab_notation.tex <==
% \begin{table}[t]
%     \centering
%     \caption{Basic Notation.}
%     \label{tab: Notation}
    
%     \begin{tabular}{ll}
%     \toprule
%     Notation& Description\\
%     \midrule
%     $W$, $H$, $D$& Spatial dimension of images (width, height and depth)\\
%     $n$& Number of stages\\ 
%     $\mathbf{I}_{m}$& Moving source images\\
%     $\mathbf{I}_{f}$& Fixed target images\\
%     $\mathbf{I}_{w}^{(k)}$& Intermediate warped registered images at stage $k$\\
%     $\mathbf{I}_{w}^{(n)}$& Final warped registered images at stage $n$\\
%     $\phi$& Deformation field - transformation between images\\
%     $\phi_L^{(k)}$& Local deformation field between $\mathbf{I}_{w}^{(k-1)}$ and $\mathbf{I}_{f}$ at stage $k$\\ 
%     $\phi_G^{(k)}$& Global deformation field between $\mathbf{I}_{m}$ and $\mathbf{I}_{f}$ at stage $k$\\ 
%     $\mathcal{T}$& Warping operation - resamples the image by given $\phi$ \\
%     \midrule
%      & Where $k=[1, \ldots, n]$\\
%     \bottomrule
%     \end{tabular}
% \end{table}

\begin{table}[t]
    \centering
    \caption{Basic Notation.}
    \label{tab: Notation}
    \vspace{-5pt}
    \begin{tabularx}{\linewidth}{lX}
    \toprule
    Notation& Description\\
    \midrule
    $W$, $H$, $D$& Spatial dimension of images (width, height and depth)\\
    $N$& Number of stages\\ 
    $\mathbf{S}$& Source images (moving)\\
    $\mathbf{T}$& Target images (fixed)\\
    $\mathbf{W}^{k}$& Intermediate warped images at stage $k$ where $k=[1, \ldots, N]$\\
    $\mathbf{W}^{N}$& Final warped registered images at stage $n$\\
    $\mathbf{\Phi}$& Deformation field - nonlinear transformation parameters between images\\
    $\mathbf{\Phi}_\text{i}^{k}$& Current deformation field between $\mathbf{W}^{k-1}$ and $\mathbf{T}$ at stage $k$ where $k=[1, \ldots, N]$\\ 
    $\mathbf{\Phi}_\text{c}^{k}$& Combined deformation field between $\mathbf{S}$ and $\mathbf{T}$ at stage $k$ where $k=[1, \ldots, N]$\\ 
    $\mathcal{T}$& Warping operation - resamples the image by given $\mathbf{\Phi}$ \\
    \bottomrule
    \end{tabularx}
    \vspace{-10pt}
\end{table}
